Coherence for rewriting 2-theories

General coherence theorems are constructed that yield explicit presentations of categorical and algebraic objects. The categorical structures involved are finitary discrete Lawvere 2-theories, though they are approached within the language of term rewriting theory. Two general coherence theorems are obtained. The first applies to terminating and confluent rewriting 2-theories. This result is exploited to construct systematic presentations for the higher Thompson groups and the Higman-Thompson groups. The presentations are categorically interesting as they arise from higher-arity analogues of the Stasheff/Mac Lane coherence axioms, which involve phenomena not present in the classical binary axioms. The second general coherence theorem holds for 2-theories that are not necessarily confluent or terminating and is used to construct a new proof of coherence for iterated monoidal categories, which arise as categorical models of iterated loop spaces and fail to be confluent.

==> titlepage.tex <==
\begin{titlepage}

\center{
      \hrule height 4pt
    \vspace{4mm}
    \huge{
    \textbf{Coherence for rewriting $2$-theories}\\
  }
 
\vspace{2mm}
 \noindent\large{\bf
    General theorems, with applications to presentations
    of Higman-Thompson groups and iterated monoidal categories.}
}
\vspace{4mm}
    \hrule height 4pt

\vspace{1in}
\center{
  \Large{\textbf{Jonathan Asher Cohen}}
}

\vspace{1in}
\center{\large{
    A thesis submitted for the degree of Doctor of Philosophy\\ of The
    Australian National University. 
}}

\vspace{1in}
\center{\large{
    June 2008
}}

\end{titlepage}

